High-Resolution Document Shadow Removal via A Large-Scale Real-World Dataset and A Frequency-Aware Shadow Erasing Net

Shadows often occur when we capture the documents with casual equipment, which influences the visual quality and readability of the digital copies. Different from the algorithms for natural shadow removal, the algorithms in document shadow removal need to preserve the details of fonts and figures in high-resolution input. Previous works ignore this problem and remove the shadows via approximate attention and small datasets, which might not work in real-world situations. We handle high-resolution document shadow removal directly via a larger-scale real-world dataset and a carefully designed frequency-aware network. As for the dataset, we acquire over 7k couples of high-resolution (2462 x 3699) images of real-world document pairs with various samples under different lighting circumstances, which is 10 times larger than existing datasets. As for the design of the network, we decouple the high-resolution images in the frequency domain, where the low-frequency details and high-frequency boundaries can be effectively learned via the carefully designed network structure. Powered by our network and dataset, the proposed method clearly shows a better performance than previous methods in terms of visual quality and numerical results. The code, models, and dataset are available at: https://github.com/CXH-Research/DocShadow-SD7K

==> tabletex/6_exp/syn.tex <==
\begin{table}[ht]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{c|ccc|ccc}
\toprule
\multirow{2}{*}{}           & \multicolumn{3}{c|}{Jung (Original)} & \multicolumn{3}{c}{Kligler (Original)} \\ \cline{2-7} 
                            & PSNR$\uparrow$    & SSIM$\uparrow$   & RMSE$\downarrow$   & PSNR$\uparrow$     & SSIM$\uparrow$   & RMSE$\downarrow$    \\ \hline
Hu \etal~\cite{hu2019mask}              & 18.99  & 0.78  & 30.38 & 25.69   & 0.88  & 15.14  \\
Hu \etal w/ Syn & 19.41  & 0.80  & 29.11 & 25.98   & 0.88  & 14.65  \\
Ours w/o Syn          & 22.21  & 0.85  & 21.37 & 24.79   & 0.92  & 15.54  \\
Ours                        & 23.53  & 0.86  & 17.65 & 29.02   & 0.93  & 10.73  \\ \bottomrule
\end{tabular}%
}
\caption{Evaluation of our shadow synthesis pipeline's effectiveness.}
\vspace{0.5em}
\label{table:syn}
\end{table}
